Analytical Second-Order Partial Derivatives of Rigid-Body Inverse Dynamics

Optimization-based robot control strategies often rely on first-order dynamics approximation methods, as in iLQR. Using second-order approximations of the dynamics is expensive due to the costly second-order partial derivatives of the dynamics with respect to the state and control. Current approaches for calculating these derivatives typically use automatic differentiation (AD) and chain-rule accumulation or finite-difference. In this paper, for the first time, we present analytical expressions for the second-order partial derivatives of inverse dynamics for open-chain rigid-body systems with floating base and multi-DoF joints. A new extension of spatial vector algebra is proposed that enables the analysis. A recursive algorithm with complexity of $\mathcal{O}(Nd^2)$ is also provided where $N$ is the number of bodies and $d$ is the depth of the kinematic tree. A comparison with AD in CasADi shows speedups of 1.5-3$\times$ for serial kinematic trees with $N> 5$, and a C++ implementation shows runtimes of $\approx$51$\mu s$ for a quadruped.

==> thebib.tex <==
\begin{thebibliography}{99}

\bibitem{tassa2012synthesis}
Y. Tassa, T. Erez and E. Todorov, "Synthesis and stabilization of complex behaviors through online trajectory optimization," in \textit{IEEE/RSJ Int.~Conf.~on Intelligent Robots and Systems}, 2012, pp. 4906-4913.

\bibitem{koenemann2015whole}
J. Koenemann et al., "Whole-body model-predictive control applied to the HRP-2 humanoid," in \textit{IEEE/RSJ Int.~Conf.~on Intelligent Robots and Systems}, 2015, pp. 3346-3351. 

\bibitem{mayne1966second}
D. Mayne, “A second-order gradient method for determining optimal trajectories of non-linear discrete-time systems,” \textit{International Journal of Control}, vol. 3, no. 1, pp. 85–95, 1966. 

\bibitem{tassa2014control}
Y. Tassa, N. Mansard, and E. Todorov, “Control-limited differential dynamic programming,” in \textit{International Conference on Robotics and Automation}, 2014. 

\bibitem{chatzinikolaidis2021trajectory}
I. Chatzinikolaidis and Z. Li, “Trajectory optimization of contact-rich motions using implicit differential dynamic programming,” \textit{IEEE Robotics and Automation Letters}, vol. 6, no. 2, pp. 2626–2633, 2021. 

\bibitem{marti2020squash}
J. Marti-Saumell, J. Sola, C. Mastalli, and A. Santamaria-Navarro, “Squash-box feasibility driven differential dynamic programming,” 2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), 2020. 

\bibitem{mastalli2020crocoddyl}
C. Mastalli, R. Budhiraja, W. Merkt, G. Saurel, B. Hammoud, et al, "Crocoddyl: An Efficient and Versatile Framework for Multi-Contact Optimal Control," in
\textit{IEEE Int.~Conf.~on Robotics and Automation}, 2020.

\bibitem{li2020hybrid}
H. Li and P. M. Wensing, “Hybrid systems differential dynamic programming for whole-body motion planning of Legged Robots,” IEEE Robotics and Automation Letters, vol. 5, no. 4, pp. 5448–5455, 2020. 

\bibitem{pellegrini2020multiple}
E. Pellegrini and R. P. Russell, “A multiple-shooting differential dynamic programming algorithm. part 1: Theory,” \textit{Acta Astronautica}, vol. 170, pp. 686–700, 2020. 

\bibitem{plancher2018performance}
B. Plancher and S. Kuindersma, “A performance analysis of parallel differential dynamic programming on a GPU,” \textit{Springer Proceedings in Advanced Robotics}, pp. 656–672, 2020. 


% \bibitem{muller}
% A. Müller and S. Kumar, “Closed-form time derivatives of the equations of motion of rigid body systems,” Multibody System Dynamics, vol. 53, no. 3, pp. 257–273, 2021. 

\bibitem{lee2005newton}
{S.-H. Lee, J.~Kim, F.~C. Park, M.~Kim, and J.~E. Bobrow, ``Newton-type
  algorithms for dynamics-based robot movement optimization,'' \emph{IEEE
  Trans.~on Robotics}, vol.~21, no.~4, pp. 657--667, 2005.}
 
  
\bibitem{nganga2021accelerating} J. N. Nganga and P. M. Wensing, “Accelerating second-order differential dynamic programming for rigid-body systems,” \textit{IEEE Robotics and Automation Letters}, vol. 6, no. 4, pp. 7659–7666, 2021. 

  \bibitem{singh2022efficient} S. Singh, R. P. Russell, and P. M. Wensing, “Efficient analytical derivatives of rigid-body dynamics using spatial vector algebra,” \textit{IEEE Robotics and Automation Letters}, vol. 7, no. 2, pp. 1776–1783, 2022. 

\bibitem{ayusawa2018comprehensive}
K. Ayusawa, E. Yoshida, "Comprehensive theory of differential kinematics and dynamics towards extensive motion optimization framework." \textit{The Int. J{.} of Robotics Research.} {vol 37(13-14), pp 1554-1572,} 2018.


\bibitem{jain1993linearization}
  A. Jain and G. Rodriguez, “Linearization of manipulator dynamics using spatial operators,” \textit{IEEE Trans.~on Systems, Man, and Cybernetics}, vol. 23, no. 1, pp. 239–248, 1993. 


\bibitem{Featherstone08}
R. Featherstone, \textit{Rigid-Body Dynamics Algorithms},
Springer, 2008.

\bibitem{garofalo2013closed}
G. Garofalo, C. Ott and A. Albu-Schäffer, "On the closed form computation of the dynamic matrices and their differentiations," in \textit{IEEE/RSJ Int.~Conf.~on Intelligent Robots and Systems}, 2013, pp. 2364-2359. 

\bibitem{andersson2019casadi}
J. A. Andersson, J. Gillis, G. Horn, J. B. Rawlings, and M. Diehl, “CasADi: A software framework for nonlinear optimization and Optimal Control,” \textit{Mathematical Programming Computation}, vol. 11, no. 1, pp. 1–36, 2018. 
\bibitem{echeandia2021numerical}
S. Echeandia, and P. M. Wensing,  "Numerical Methods to Compute the Coriolis Matrix and Christoffel Symbols for Rigid-Body Systems." ASME. J. Comput. Nonlinear Dynam. September 2021; 16(9): 091004.

\bibitem{sola}
J. Solà, J. Deray, D. Atchuthan, A micro Lie theory for state estimation in robotics
, \textit{ArXiv}, vol. 	abs/1812.01537, 2018.

\bibitem{arxivss}
S. Singh, R. Russell, P. Wensing, Efficient Analytical Derivatives of Rigid-Body Dynamics using Spatial Vector Algebra
, \textit{ArXiv}, vol. 	abs/2105.05102, 2021.

\bibitem{arxivss_SO}
S. Singh, R. Russell, P. Wensing, Details of Partial Derivatives of Rigid-Body Inverse Dynamics
, \textit{ArXiv}, vol. 	abs/2105.05102, 2022.



% \bibitem{carpentier}
% J. Carpentier, N. Mansard, "Analytical Derivatives of Rigid-Body Dynamics Algorithms," in \textit{Robotics: Science and Systems},  Pittsburgh, United States, Jun. 2018.

\bibitem{carpentier2019pinocchio}
J. Carpentier, G. Saurel, G. Buondonno, J. Mirabel, F. Lamiraux, O. Stasse, and N. Mansard, “The pinocchio C++ library : A fast and flexible implementation of rigid body dynamics algorithms and their analytical derivatives,”  \textit{IEEE/SICE International Symposium on System Integration (SII)}, 2019. 

\bibitem{eigen}
G. Guennebaud, B. Jacob, en Others, “Eigen v3”, 2010. [Online]. Available at: http://eigen.tuxfamily.org.

% \bibitem{ctmm2}
% V. Samy, K. Ayusawa ,E. Yoshida, "Generalized Comprehensive Motion Theory for High-Order Differential Dynamics," in \textit{Robotics: Science and Systems}, Jul. 2021.



% \bibitem{jong}
% J. J. de Jong, A. Müller, and J. L. Herder, “Higher-order derivatives of rigid body dynamics with application to the dynamic balance of spatial linkages,” \textit{Mechanism and Machine Theory}, vol. 155, p. 104059, 2021. 


% \bibitem{niemeyer1991performance}
% G. Niemeyer, J.-J. E. Slotine "Performance in Adaptive Manipulator Control," \textit{The International Journal of Robotics Research}, vol 10, no. 2, pp 149-161, 1991.

\bibitem{matlabsource}
\url{https://github.com/ROAM-Lab-ND/spatial_v2_extended}





\end{thebibliography}
